Mathematical Modeling of Cyber Resilience

We identify quantitative characteristics of responses to cyber compromises that can be learned from repeatable, systematic experiments. We model a vehicle equipped with an autonomous cyber-defense system and which also has some inherent physical resilience features. When attacked by malware, this ensemble of cyber-physical features (i.e., "bonware") strives to resist and recover from the performance degradation caused by the malware's attack. We propose parsimonious continuous models, and develop stochastic models to aid in quantifying systems' resilience to cyber attacks.

==> includes/20-prior-work.tex <==
\section{Prior work}\label{sec:prior-work}

A growing body of literature explores quantification of resilience in general and cyber resilience in particular. Very approximately, the literature can be divided into two categories: 
(1) qualitative assessments of a system (actually existing or its design) by subject matter experts (SMEs) \cite{alexeev}, \cite{henshel} and 
(2) quantitative measurements based on empirical or experimental observations of how a system (or its high-fidelity model; \cite{kott2017assessing}) responds to a cyber compromise \cite{kott2019cyber,ligo2021how}.
In the first category, a well-cited example is the approach called the cyber-resilience matrix \cite{linkov2013resilience}. In this approach, a system is considered as spanning four domains: (1) physical (i.e., the physical resources of the system, and the design, capabilities, features and characteristics of those resources); (2) informational (i.e., the system's availability, storage, and use of information); (3) cognitive (i.e., the ways in which informational and physical resources are used to comprehend the situation and make pertinent decisions); and (4) social (i.e., structure, relations, and communications of social nature within and around the system). For each of these domains of the system, SMEs are asked to assess, and to express in metrics, the extent to which the system exhibits the ability to (1) plan and prepare for an adverse cyber incident; (2) absorb the impact of the adverse cyber incident; (3) recover from the effects of the adverse cyber incident; and (4) adapt to the ramifications of the adverse cyber incident. In this way, the approach defines a 4-by-4 matrix that serves as a framework for structured assessments by SMEs.     

Another example within the same category (i.e., qualitative assessments of a system by SMEs) is a recent, elaborate approach proposed by \cite{beling2021developmental}. The approach is called Framework for Operational Resilience in Engineering and System Test (FOREST), and a key methodology within FOREST is called Testable Resilience Efficacy Elements (TREE). For a given system or subsystem, the methodology requires SMEs to assess, among others, how well the resilience solution is able to (1) sense or discover a successful cyber-attack; (2) identify the part of the system that has been successfully attacked; (3) reconfigure the system in order to mitigate and contain the consequences of the attack. Assessment may include tests of the system, although the methodology does not prescribe the tests. 

Undoubtedly, such methodologies can be very valuable in finding opportunities in improvements of cyber-resilience in a system that is either at the design stage or is already constructed. Still, these are essentially qualitative assessments, not quantitative measurements derived from an experiment. 

In the second category (i.e., quantitative measurements based on empirical or experimental observations of how a system, or its high-fidelity model, responds to a cyber compromise), most approaches tend to revolve around a common idea we call here the area under the curve (AUC) method \cite{hosseini2016review,kott2021to}.
%The general idea is depicted in Figure~\ref{fig:auc}.
In an experiment/test, a system is engaged into a performance of a representative mission, and then is subjected to an ensemble or sequence of representative cyber attacks. A mission-relevant quantitative functionality of the system is observed and recorded. The resulting average functionality, divided by normal functionality, can be used as a measure of resilience.  

%%%%% \begin{figure}[t]
%%%%%   \centering
%%%%%   %\includegraphics[width=\columnwidth]{attacks_and_defenses.pdf}
%%%%%   \aaa{attacks_and_defenses.pdf}
%%%%%   \caption{Resilience can be measured by subjecting a system to cyber attacks %%%%%  and measuring the fraction of functionality lost due to cyber attack, as %%%%%  compared to normal functionality.}
%%%%%   \label{fig:auc}
%%%%% \end{figure}

Brtis \cite{brtis2016how} performed a structured evaluation and comparison of multiple resilience metrics and concluded that the AUC-based approaches are superior to others. He wrote, ``We evaluated 23 candidate metrics against 19 evaluation criteria. From this analysis we conclude that the best single metric for resiliency is the expected availability of the required capability.'' Parenthetically, our research did not find a reason to disagree with Brtis's position. 

However, AUC-based resilience measures are inherently cumulative, aggregate measures, and do not tell us much about the underlying processes. For example, is it possible to quantify the resilience \impact{} of the bonware of the given system? Similarly, is it possible to quantify the \impact{} of malware? In addition, is it possible to gain insights into how these values of \impact{fulness} vary over time during an incident? We offer steps toward answering such questions.  

==> includes/20-prior-work_w_fig_1_included.tex <==
\section{Prior work}\label{sec:prior-work}

A growing body of literature explores quantification of resilience in general and cyber resilience in particular. Very approximately, the literature can be divided into two categories: 
(1) qualitative assessments of a system (actually existing or its design) by subject matter experts (SMEs) \cite{alexeev}, \cite{henshel} and 
(2) quantitative measurements based on empirical or experimental observations of how a system (or its high-fidelity model; \cite{kott2017assessing}) responds to a cyber compromise \cite{kott2019cyber,ligo2021how}.
In the first category, a well-cited example is the approach called the cyber-resilience matrix \cite{linkov2013resilience}. In this approach, a system is considered as spanning four domains: (1) physical (i.e., the physical resources of the system, and the design, capabilities, features and characteristics of those resources); (2) informational (i.e., the system's availability, storage, and use of information); (3) cognitive (i.e., the ways in which informational and physical resources are used to comprehend the situation and make pertinent decisions); and (4) social (i.e., structure, relations, and communications of social nature within and around the system). For each of these domains of the system, SMEs are asked to assess, and to express in metrics, the extent to which the system exhibits the ability to (1) plan and prepare for an adverse cyber incident; (2) absorb the impact of the adverse cyber incident; (3) recover from the effects of the adverse cyber incident; and (4) adapt to the ramifications of the adverse cyber incident. In this way, the approach defines a 4-by-4 matrix that serves as a framework for structured assessments by SMEs.     

Another example within the same category (i.e., qualitative assessments of a system by SMEs) is a recent, elaborate approach proposed by \cite{beling2021developmental}. The approach is called Framework for Operational Resilience in Engineering and System Test (FOREST), and a key methodology within FOREST is called Testable Resilience Efficacy Elements (TREE). For a given system or subsystem, the methodology requires SMEs to assess, among others, how well the resilience solution is able to (1) sense or discover a successful cyber-attack; (2) identify the part of the system that has been successfully attacked; (3) reconfigure the system in order to mitigate and contain the consequences of the attack. Assessment may include tests of the system, although the methodology does not prescribe the tests. 

Undoubtedly, such methodologies can be very valuable in finding opportunities in improvements of cyber-resilience in a system that is either at the design stage or is already constructed. Still, these are essentially qualitative assessments, not quantitative measurements derived from an experiment. 

In the second category (i.e., quantitative measurements based on empirical or experimental observations of how a system, or its high-fidelity model, responds to a cyber compromise), most approaches tend to revolve around a common idea we call here the area under the curve (AUC) method \cite{hosseini2016review,kott2021to}. The general idea is depicted in Figure~\ref{fig:auc}. In an experiment/test, a system is engaged into a performance of a representative mission, and then is subjected to an ensemble or sequence of representative cyber attacks. A mission-relevant quantitative functionality of the system is observed and recorded. The resulting average functionality, divided by normal functionality, can be used as a measure of resilience.  

\begin{figure}[t]
  \centering
  %\includegraphics[width=\columnwidth]{attacks_and_defenses.pdf}
  \aaa{attacks_and_defenses.pdf}
  \caption{Resilience can be measured by subjecting a system to cyber attacks and measuring the fraction of functionality lost due to cyber attack, as compared to normal functionality.}
  \label{fig:auc}
\end{figure}

Brtis \cite{brtis2016how} performed a structured evaluation and comparison of multiple resilience metrics and concluded that the AUC-based approaches are superior to others. He wrote, ``We evaluated 23 candidate metrics against 19 evaluation criteria. From this analysis we conclude that the best single metric for resiliency is the expected availability of the required capability.'' Parenthetically, our research did not find a reason to disagree with Brtis's position. 

However, AUC-based resilience measures are inherently cumulative, aggregate measures, and do not tell us much about the underlying processes. For example, is it possible to quantify the resilience \impact{} of the bonware of the given system? Similarly, is it possible to quantify the \impact{} of malware? In addition, is it possible to gain insights into how these values of \impact{fulness} vary over time during an incident? We offer steps toward answering such questions.  

==> includes/32-cyber-resilience.tex <==
\subsection{Cyber resilience}

In Section~\ref{sec:prior-work} we discussed a measure of cyber resilience, the area under the functionality curve, which is precisely the mission accomplishment $\ma(T)$ evaluated at the final time of the mission.  To be able to compare measures of cyber resilience for multiple missions, we normalize the measure by dividing by the total mission time.
\begin{equation*}
  R= \frac{1}{T-t_0} \int_{t_0}^T \functionality(\tau) \, d\tau =
  \frac{\ma(T)}{T-t_0}.
\end{equation*}
Often there are multiple objectives to a mission.  Given a vector of resiliences, $\mathbf{R} =(R_1,R_2, \hdots, R_n),$ we define the overall cyber resilence to be the
root-mean-square resilience of our mission:
\begin{eqnarray*}
  R= ||\mathbf{R}||_2 
  %&=& \sqrt{\sum_{j=1}^n R_j^2} \\
  =
  \frac{1}{T-t_0}
  \sqrt{
    \sum_{j=1}^n
    \left( \int_{t_0}^T \functionality_j(\tau) \, d\tau \right)^2}.
\end{eqnarray*}
\normalsize
Because each mission accomplishment may have a different relative importance, we may account for this by weighting the normal functionalities ${\Fnominal}_j$.  To enforce an overall mission resilience in the range $[0,1]$, we renormalize to obtain normalized resilience $\mathcal{R}$.
\begin{equation*}
  \mathcal{R} = \frac{R}{\left( \sum_{j=1}^n {\Fnominal}_j^2\right)^{1/2} }.
\end{equation*}



==> includes/40-continuous-model.tex <==
\section{Continuous model}\label{sec:continuous}

For the first set of models, we make the assumption that mission accomplishment is twice continuously differentiable: $\ma\in C^2$, and thus $\functionality \in C^1$. 

As a first approximation, we let the \impact{} of malware on the
derivative of functionality be linear:
$\frac{d\functionality_m(t)}{dt} = - \functionality(t) \malware(t)$.
The \impact{} of bonware is similarly defined and proportional to the
level of functionality below normal.
$\frac{d\functionality_b(t) } {dt} = (\Fnominal-F(t)) \bonware(t)$.
Malware degrades the system while bonware aims to increase
functionality over time.  Malware \impact{} and bonware \impact{} are
assumed to be continuous functions of time,
$\malware, \bonware \in C^0.$ The \impact{} on functionality is the sum
of the \impact{s} of malware and bonware:
$\frac{d\functionality(t)}{dt} = \frac{d\functionality_m(t)}{dt} +
\frac{d\functionality_b(t)}{dt}$. Then
\begin{equation}
  \frac{d\functionality}{dt} = (\Fnominal-\functionality(t)) \bonware(t) - \functionality(t) \malware(t).
\label{eq:0}
\end{equation}
Since we expect bonware to help (or at least not harm) and malware to
not help, we assume $\bonware(t) \ge 0$ and $\malware(t) \ge 0$ and we
let $\Qware(t)=\malware(t)+\bonware(t).$ We also assume normal
functionality is positive, $\functionality_0 > 0,$ and functionality
is always nonnegative and less than or equal to normal functionality,
$0 \le \functionality(t) \le \Fnominal.$ Equation~\ref{eq:0} can be
written as
\begin{equation}
  \frac{d\functionality}{dt} + \Qware(t) \functionality(t) = \Fnominal \bonware (t).
\label{eq:00}
\end{equation}
This first-order linear differential equation has the following solution: 
\begin{equation}
  F(t)  = \expminus \left( F(0) + \bintegral \right).
\end{equation}
%%% \begin{equation*}
%%% \frac{\functionality(t)}{\Fnominal} =
%%% e^{- \int_0^t \Qware(p) \, dp} \int_0^t  \bonware(\tau)
%%% e^{\int_0^\tau \Qware(p) \, dp} \, d\tau.  
%%% \end{equation*}
%%% %%%
%%% Letting
%%% \begin{equation*}
%%%   \begin{aligned}
%%%     \malware(t) &=E_m(t) A_m(t),\\
%%%     \bonware(t) &=E_b(t) A_b(t),\\
%%%     \Qware(t)    &= E_m(t) A_m(t)+E_b(t) A_b(t) ,
%%%   \end{aligned}
%%% \end{equation*}
To help us understand how the model works, we find explicit solutions for a number of examples.  We start with a piecewise constant malware \impact{}, piecewise constant bonware \impact{}, and also look at a piecewise linear model.  




==> includes/42-piecewise-constant-model.tex <==
\subsection{Piecewise constant model}

If either malware's or bonware's impact diminishes at some point in the incident, the model may switch from one set of constants defining malware and bonware to another set of constants.  The differential equation (Eq.~\ref{eq:0}) may now be expressed as
\begin{equation}
  \frac{d\functionality}{dt} = \sum_{j=0}^{N-1}(\Fnominal-\functionality(t)) \bonware_j(t) -  \functionality(t) \malware_j (t),
  \label{eq:000}
\end{equation}
where the vectors $\boldsymbol{\malware} =( {\malware}_0, {\malware}_1, \cdots {\malware}_{N-1} )$ and $\boldsymbol{\bonware} =( {\bonware}_0,  {\bonware}_1,\cdots, {\bonware}_{N-1})$ contain the malware \impact{} and bonware \impact{}s within time windows whose end points are defined by  $\{t_0, t_1, \cdots, t_N \}$. The solution will be a function which, in each time interval, is the solution found in Equation~\ref{eq:3}:
\begin{align*} \label{eq:piecewise:constant}
    \functionality(t)     = \left[\functionality(t_j) - \frac{\Fnominal \bonware_j}{ \Qware_j }
    \right] e^{-\Qware_j\cdot (t-t_j)} + \frac{\Fnominal \bonware_j}{\Qware_j},\\
    \quad (t_j \le t < t_{j+1}), \quad (j=0,\cdots, N-1)
\end{align*}
where $\Qware_j = \malware_j + \bonware_j$.  The smooth line in Figure~\ref{fig:notional} is an example realization of this model.
% -----------------------------------------------------------------
% The figure is referenced here, so we place it here ...
% (moved from 70-application-of-model.tex )
% -----------------------------------------------------------------
\begin{figure}[h]
  \centering
  % \aaa{curves.pdf}
  \aaa{curves_rescaled.pdf}
  \caption{The smooth line is an example functionality curve with piecewise constant malware and bonware impacts.  The notional data and piecewise constant model fit are described below in Section \ref{sec:parameters}.}
  \label{fig:notional}
\end{figure}


==> includes/44-piecewise-linear-models.tex <==
\subsection{Piecewise linear model}

\newcommand{\tcj}{\Omega_j(t)}
\newcommand{\td}{\Lambda}

Both malware and bonware \impact{}s may initially be linear, but if
the situation changes and a different linear model holds after a time,
the model should be able to account for it.  In particular, if malware
\impact{} is decreasing over time, at some point we will reach
$\malware=0$ and the model switches to a new linear model.
Equation~\ref{eq:linear:model} can be written
\begin{equation*}
  \frac{d\functionality}{dt} = \sum_{j=0}^{N-1}  \left[ (\lambda_j - \omega_j t) \functionality(t) -  \Fnominal (\alpha_j - \beta_j t) \right]. \label{eq:piecewise:linear}
\end{equation*}
The solution follows from Equation~\ref{eq:6}:
\begin{align*} \label{eq:piecewise:linear:solution}
  \frac{\functionality(t)}{\Fnominal} &= \frac{1}{\tcj} 
  \left\{ 
    \frac{\functionality(t_j)}{\Fnominal}-\frac{\beta_j}{\omega_j }\left(1-\tcj\right) +(\alpha_j  \omega_j -\beta_j  \lambda_j )\right.\\
  \times & \left. \frac{\sqrt{\frac{\pi }{2}} e^{\td_j^2 }}{\omega_j^{3/2}} \left[\text{erf}\left(\td_j\right)+\text{erf}\left(\frac{\omega_j (t-t_j) }{\sqrt{2 \omega_j }}-\td_j\right)\right] \right\},\\
& \quad (t_j \le t < t_{j+1}), \quad (j=0,\cdots, N-1)
\end{align*}
where $\tcj=e^{\lambda_j (t-t_j)-\frac{1}{2}\omega_j (t-t_j)^2 }$ and $\td_j=\sfrac{\lambda_j }{\sqrt{2 \omega_j }}$.  

Example realizations of the piecewise linear models are shown in Figure~\ref{fig:piecewise:linear}.

\begin{figure}[th]
  \centering
%    \aaa{figure_3.pdf}
    \aaa{figure_3_rescaled.pdf}
    \caption{Normalized functionality, $\functionality(t)/\Fnominal$, is shown for piecewise linear models. Both malware and bonware \impact{}s are initially linear functions of time.  When malware \impact{} reaches $\malware=0$, then malware \impact{} is zero but bonware \impact{} continues to increase.}
    \label{fig:piecewise:linear}
\end{figure}

==> includes/53-interaction-sde.tex <==
\subsection{Interaction between bonware and malware}

In all previous models, bonware and malware have acted independently from one another, increasing and decreasing functionality respectively.  In the next version of the model, we additionally allow bonware to act on malware rather than only on functionality directly.  This requires the introduction of an interaction term $\bonwareInteraction$ incorporated in the generic model of Equation~\ref{eq:sde:generic}:
$$\frac{d \functionality}{d t} 
  =  \left(1-\functionality(t)\right) \bonwareActivity \bonwareEffectiveness\nonumber-\functionality(t) \malwareActivity \malwareEffectiveness \bonwareInteraction.$$

To complete the interaction model, we may specify that $\bonwareInteraction = \unitstep\!\left(\tint-t\right)$, so that the malware has its regular effect until some time $\tint$, when the malware retreats or is disabled by the bonware. Figure~\ref{fig:psdel} (left) shows simulated data from this model with $\bonwareRate=0.12$, $\bonwareSize=0.71$, $\malwareRate=0.08$, and $\malwareSize=0.34$.

==> includes/54-linear-sde.tex <==
\subsection{Gradually changing parameters}\label{sec:sde:gradual}

In a final variation of the SDE model, we allow parameters $\bonwareActivity$ and $\malwareActivity$ to evolve gradually over time.  A possible application of such a model is the scenario in which malware and bonware actively explore weaknesses and their probability of success may increase over time.  A simulated example of a functionality curve in such a scenario is give in Figure~\ref{fig:psdel} (right).  The functionality shows a period of decrease during the initial period of attack, then a period of high variability as both malware and bonware are active, and a period of recovery after the conclusion of the attack.  
Underlying this pattern is the bonware activity that gradually increases, $\bonwareActivity = \Phi(at+b)$, and malware activity that gradually increases until it is turned off at time $\tint$, $\malwareActivity = \Phi(ct+d)\unitstep(\tint-t)$, where % $\Phi(\cdot)$ is the cumulative density function of the standard normal distribution. 
\blue{$\Phi(z)=\frac{1}{2}+\frac{1}{2} \erf{(\frac{z}{\sqrt{2}})}$}{} is the cumulative density function of the standard normal distribution. 

% \begin{figure*}[bh]
\begin{figure*}[ht]
\centering
%\includegraphics[width=\columnwidth]{figures/piecewise_stochastic_step_with_interaction-sim.pdf}
%\includegraphics[width=\columnwidth]{figures/piecewise_stochastic_step_linear_parameters-sim.pdf}
\ppp{figures/piecewise_stochastic_step_with_interaction-sim-small.pdf}
\qqq{figures/piecewise_stochastic_step_linear_parameters-sim-small.pdf}

    \caption{\textbf{Left:} Simulated data from the SDE model with interaction between bonware and malware.  The angular blue-grey line depicts functionality over mission time.  Changes in functionality occur at random intervals and random step sizes.  The red line and downward pointing marker indicate the period during which malware is active.  This period permits downward steps in functionality.  The green line and upward pointing marker indicate period during which bonware is active.  This period permits upward steps in functionality.  The red marker indicates the onset of a cyber attack and the green marker indicates its conclusion. \textbf{Right:} Simulated data from the SDE model with gradually changing parameters.  Here, the probability that an attack will harm functionality is depicted as a smooth orange curve.  The probability increases over mission time until the attack is repelled.  The smooth purple curve indicates the probability that a bonware attempt to restore functionality is successful. As the smooth curves rise, the rate of steps in the functionality curve increases.  Data were simulated from the equations in Section~\ref{sec:sde:gradual} with $a=0.063$, $b=-6.0$, $c=0.025$, $d=-1.5$.}
    \label{fig:psdel}
\end{figure*}

==> includes/70-application-of-model.tex <==
\section{An application of the model}
\subsection{Obtaining model parameters}
\label{sec:parameters}
%
% ----------------------------------------------------------------
% We reference this figure earlier, so moved it to 42-piecewise-constant-model.tex
% ----------------------------------------------------------------
% \begin{figure}[htbp]
%%%  \begin{figure}[h]
%%%    \centering
%%%    \aaa{curves.pdf}
%%%    \caption{The notional data and piecewise-constant malware/bonware model fit.}
%%%    \label{fig:notional}
%%%  \end{figure}
%
Given notional data that represents a typical curve of functionality
over the course of an incident where malware and bonware are active,
we develop a fast method to estimate the continuous model parameters
for a curve that approximates the data, and use these parameters to
generate further realizations based on this model.  In Figure
\ref{fig:notional} an example of such notional data is plotted (in
light blue/gray).  In this section, we illustrate our method to
extract the model parameters from this curve.

%%% Given the plotted (light blue/gray) notional data in Figure \ref{fig:notional}, we seek to fit a curve conforming to the piecewise-constant malware/bonware model so that we can extract the model parameters and produce new realizations of curves from this model.  

% Recall, the piecewise-constant malware/bonware model (which we will henceforth refer to as ``Continuous Model I''), assumes both malware and bonware are constant over each of a finite number of intervals.   The parameters  $\malwareEffectivenessConstant$ and $A_m$ are the malware effectiveness and malware activity, and the parameters $E_b$ and $\bonwareActivityConstant$ are the bonware effectiveness and activity.

The set $P=\{t_0, \hdots, t_K\}$ partitions the mission timeline and
malware and bonware are constant in each interval $(t_{i-1},t_i), \,\,
i=1, \hdots, K. \,\,$  In each interval,
$\Qware_i=\malware_i+\bonware_i$ and the differential equation
governing Continuous Model I is $\frac{dF(t)}{dt}+\Qware_i F(t) =
\Fnominal (t) \bonware_i.$  Thus, in each interval $(t_{i-1},t_i),$
the solution is 
\begin{equation*}
  \functionality(t)     =
  \left[\functionality(t_{i-1}) - \frac{\Fnominal \bonware_i}{
      \Qware_i } \right]  e^{-\Qware_i (t-t_{i-1})} + \frac{\Fnominal \bonware_i}{\Qware_i}.
\end{equation*}
We compute the effectiveness, $\malwareEffectivenessConstant$, and activity, $\malwareActivityConstant$, of malware
and of bonware ($\bonwareEffectivenessConstant, \bonwareActivityConstant$), in each interval:
$\malware_i = \malwareEffectivenessConstant_i \malwareActivityConstant_i$, $\bonware_i = \bonwareEffectivenessConstant_i \bonwareActivityConstant_i$.
% Given the task of fitting a piecewise model to our notional data,

We observe that there is a unique switching time $\tchange$ where the
functionality's trend reverses, and thus we take $K=2.$ Before the
switch, the impact of malware is greater than that of bonware. From
the time of the switch until the end of the mission, bonware is
stronger.  To estimate the switching time $\tchange$, we find the
minimum of the data to occur over the interval from 64 s to 75 s.
There, the minimum value of the data curve is $m=0.27$.  Taking the
midpoint, our estimate for $\tchange$ is 69.5 s.  We estimate the
activity of malware before switching to be the number of times the
data curve decreases divided by the switching time.  Similarly, our
estimate of bonware activity is the number of times the data curve
increases prior to the switching time.  We thus have
$\malwareActivityConstant_1~\approx~\sfrac{7}{69.5}~\approx 0.101$ and
$\bonwareActivityConstant_1 \approx \sfrac{2}{69.5} \approx 0.014$.


To determine the remaining parameters, we numerically solve this system of equations:
\begin{align*}
    \alpha m & = \Fnominal \bonQone,\\
    m & = \functionality(0)  -\Fnominal \bonQone e^{-\Qware_1 \tchange}+\Fnominal \bonQone.
\end{align*}
The first equation says that where the curve meets the minimum of the data, it has experienced exponential decay of $\alpha$ toward the asymptotic minimum.  We take $\alpha$ to be $\alpha=1-\sfrac{1}{e}$. The second equation says that the minimum occurs at the switching time (the time when the model switches from malware dominating bonware, to bonware dominating malware.  Solving this system of equations yields (with $\malware_1=\Qware_1-\bonware_1$), $\malware_1 \approx  0.025$ and $\bonware_1 \approx 0.005$, so that $\malwareEffectivenessConstant_1 = \sfrac{\malware_1}{\malwareActivityConstant_1} \approx 0.503$ and $\bonwareEffectivenessConstant_1 = \sfrac{\bonware_1}{\bonwareActivityConstant_1}\approx 0.362$.

To the right of $t^\star$, we fit an exponentially increasing function.  Similar to before the switching time, we compute the activities of the malware and bonware: $\malwareActivityConstant_2 \approx \frac{1}{100-69.5} \approx 0.033$ and $\bonwareActivityConstant_2 \approx \frac{4}{100-69.5} \approx 0.131$.

To determine the remaining parameters, we numerically solve this system of equations:
  \begin{align*}
    \zeta & = F(0)   \bonQtwo,\\
    \tilde{\alpha} \zeta & = \left(m-\Fnominal
    \bonQtwo\right)\left(e^{-\Qware_2 (125-t^\star)}+\Fnominal \bonQtwo\right).
  \end{align*}
  
We have found that $\tilde{\alpha}=1-e^{-4}$ and $\zeta=0.95$ are
satisfactory values to use for these hyperparameters.

We compute $\malware_2 \approx  0.005$ and $\bonware_2 \approx 0.088$, so that $\malwareEffectivenessConstant_1 = \sfrac{\malware_1}{\malwareActivityConstant_1} \approx 0.201$ and $\bonwareEffectivenessConstant_1 = \sfrac{\bonware_1}{\bonwareActivityConstant_1}\approx 0.957$.

  

% \renewcommand\tableintroline[3]{#1 & #2 & #3 \\ \hline}
% \renewcommand\tableline[3]{$#1$ & #2 & #3 \\ \hline}
% \begin{table*}[!t]
% % \caption{System parameters used to compute bit error rate.}
%  \caption{Parameters used in our analysis.}
%   \label{table:one}
%   \centering
%   \begin{tabular}{|c|l|c|}
%     \hline \tableintroline{Symbol}{Description}{Range of Values} \hline
%       %-----------------------------------------------------------------
%       \tableline{F_0}{Nominal Functionality}{$(0,\infty)$}
%       \tableline{F}{Functionality}{$[0,F_0]$}
%       \tableline{\malware}{Malware \Impact}{[0,1]}
%       \tableline{\bonware}{Bonware \Impact}{[0,1]}
%       \tableline{\Qware}{Sum of Malware and Bonware \Impact{}s}{[0,2]}
%       % \tableline{\malwareActivityConstant}{Activity of Malware}{[0,1]}
%       % \tableline{\bonwareActivityConstant}{Activity of Bonware}{[0,1]}
%       % \tableline{E_m}{Effectiveness of Malware}{[0,1]}
%       % \tableline{E_b}{Effectiveness of Bonware}{[0,1]}
%       %-----------------------------------------------------------------
%   \end{tabular}
% \end{table*}

% \begin{table*}[!t]
% % \caption{System parameters used to compute bit error rate.}
%  \caption{Estimated Values.}
%   \label{table:two}
%   \centering
%   \begin{tabular}{|c|l|c|}
%     \hline \tableintroline{Symbol}{Description}{Computed Value} \hline
%       %-----------------------------------------------------------------
%       \tableline{t^\star}{Switching time [seconds]}{69.5}
%     \tableline{F(t^\star)}{Minimum of functionality }{0.27}
%     \hline
%       \tableline{{\malwareActivityConstant}_1}{Activity of Malware prior to time $t^\star$}
%                                     {0.100719}
%       \tableline{{\bonwareActivityConstant}_1}{Activity of Bonware prior to time $t^\star$}
%                           {0.143885}
%       \tableline{{E_m}_1}{Effectiveness of Malware prior to time $t^\star$}
%                 {0.502855}
%       \tableline{{E_b}_1}{Effectiveness of Bonware prior to time $t^\star$}
%                           {0.3622}
%       %-----------------------------------------------------------------
%     \hline
%     \tableline{{\malwareActivityConstant}_2}{Activity of Malware for $t \ge t^\star$}
%                                     {0.0327869}
%       \tableline{{\bonwareActivityConstant}_2}{Activity of Bonware for $t \ge t^\star$}
%                           {0.131148}
%       \tableline{{E_m}_2}{Effectiveness of Malware for  $t \ge t^\star$}
%                 {0.201455}
%       \tableline{{E_b}_2}{Effectiveness of Bonware for $t \ge t^\star$}
%                           {0.956862}
%       %-----------------------------------------------------------------
%   \end{tabular}
% \end{table*}

\subsection{Generating stochastic realizations}

Using the parameters found in Section~\ref{sec:parameters}, we can now
generate stochastic realizations.  In Section~\ref{sec:proposition},
we showed that for large sample sizes, the average of our ensemble
will approach the solution to the continuous ODE model.  We show
empirically that this is indeed the case.  To illustrate, we generated
five realizations (Figure \ref{fig:five:realizations}) of the
stochastic model with parameters found from the notional data of
Section~\ref{sec:parameters}.  We averaged these curves to obtain the
$n=5$ curve in Figure~\ref{fig:average}.  By averaging $n$ curves when
$n \in \{5,50,500,5000\}$ we see how the ensemble average approaches
the solution of the corresponding differential equation as predicted
in the Theorem of Section~\ref{sec:proposition}.

\begin{figure}[ht]
\begin{center}
%   \aaa{five_realizations.pdf}
   \aaa{five_realizations_reduced.pdf}
 \caption{Five realizations of the stochastic model generated with the
   parameters obtained by fitting the notional data shown in Figure
   \ref{fig:notional}.  Each realization is different but each roughly follows
   an exponential decay when $t<t^\star=69.5$ s and an
   exponential recovery for $t\ge t^\star$. }
   \label{fig:five:realizations}
 \end{center}
 \end{figure}

\begin{figure}[ht]
  \centering
  %  \aaaaaa{avg_over_n_runs.pdf}
%   \aaa{stochastic_averaging.pdf}
  \aaa{stochastic_averaging_reduced.pdf}
  \caption{Averages of $n$ stochastic runs for $n\in \{5,50,500,5000\}.$  As $n$ increases, the average of the ensemble approaches the fitted curve as predicted in the theorem of Section \ref{sec:proposition}. }
  \label{fig:average}
\end{figure}

